Data-Agnostic Augmentations for Unknown Variations: Out-of-Distribution Generalisation in MRI Segmentation

Medical image segmentation models are often trained on curated datasets, leading to performance degradation when deployed in real-world clinical settings due to mismatches between training and test distributions. While data augmentation techniques are widely used to address these challenges, traditional visually consistent augmentation strategies lack the robustness needed for diverse real-world scenarios. In this work, we systematically evaluate alternative augmentation strategies, focusing on MixUp and Auxiliary Fourier Augmentation. These methods mitigate the effects of multiple variations without explicitly targeting specific sources of distribution shifts. We demonstrate how these techniques significantly improve out-of-distribution generalization and robustness to imaging variations across a wide range of transformations in cardiac cine MRI and prostate MRI segmentation. We quantitatively find that these augmentation methods enhance learned feature representations by promoting separability and compactness. Additionally, we highlight how their integration into nnU-Net training pipelines provides an easy-to-implement, effective solution for enhancing the reliability of medical segmentation models in real-world applications.

==> figures/esoteric/pca_acdc_avg_transformed.tex <==

\definecolor{backg}{RGB}{42, 179, 205}
\definecolor{myo}{RGB}{250, 231, 35}
\definecolor{leftv}{RGB}{253, 127, 116}
\definecolor{rightv}{RGB}{150, 55, 173}
\begin{tikzpicture}
    \pgfplotstableread[col sep=comma]{figures/esoteric/pca/acdc/No_Aug_esoteric_depth_0_pca.csv}\datatable
\begin{axis}[width=0.20\textwidth,
            xmin=-8,xmax=8,
            ymin=-8,ymax=8,
, xtick={-5,0,5}, ytick={-5,0,5}
]
    \addplot[
        scatter/classes={0={backg}, 1={leftv}, 2={myo}, 3={rightv}},
        scatter, mark=*, only marks, 
        mark options={xscale=0.5pt, yscale=0.5pt},
        scatter src=explicit symbolic,
        % nodes near coords*={\Label},
        visualization depends on={value \thisrow{label} \as \Label} %<- added value
    ] table [x index = 0, y index = 1, meta=label] {\datatable};
\end{axis}
\node[above,font=\scriptsize] at (current bounding box.north) {\hspace{4ex} No Aug. (-0.138)};
\end{tikzpicture}%
\begin{tikzpicture}
    \pgfplotstableread[col sep=comma]{figures/esoteric/pca/acdc/Base_esoteric_depth_0_pca.csv}\datatable
\begin{axis}[width=0.20\textwidth, xmin=-5,xmax=10,ymin=-5,ymax=5,                         xtick={-5,0,5,10},             ytick={-4,0,4}]
    \addplot[
        scatter/classes={0={backg}, 1={leftv}, 2={myo}, 3={rightv}},
        scatter, mark=*, only marks, 
        mark options={xscale=0.5pt, yscale=0.5pt},
        scatter src=explicit symbolic,
        % nodes near coords*={\Label},
        visualization depends on={value \thisrow{label} \as \Label} %<- added value
    ] table [x index = 0, y index = 1, meta=label] {\datatable};
\end{axis}
\node[above,font=\scriptsize] at (current bounding box.north) {\hspace{4ex} Base (0.074)};
\end{tikzpicture}%
\begin{tikzpicture}
    \pgfplotstableread[col sep=comma]{figures/esoteric/pca/acdc/MixUp_esoteric_depth_0_pca.csv}\datatable
\begin{axis}[width=0.20\textwidth, xmin=-4,xmax=6,ymin=-5,ymax=5,                         xtick={-4,0,4},             ytick={-4,0,4}]
    \addplot[
        scatter/classes={0={backg}, 1={leftv}, 2={myo}, 3={rightv}},
        scatter, mark=*, only marks, 
        mark options={xscale=0.5pt, yscale=0.5pt},
        scatter src=explicit symbolic,
        % nodes near coords*={\Label},
        visualization depends on={value \thisrow{label} \as \Label} %<- added value
    ] table [x index = 0, y index = 1, meta=label] {\datatable};
\end{axis}
\node[above,font=\scriptsize] at (current bounding box.north) {\hspace{4ex} + MixUp (0.106)};
\end{tikzpicture}%
\begin{tikzpicture}
    \pgfplotstableread[col sep=comma]{figures/esoteric/pca/acdc/AFA_esoteric_depth_0_pca.csv}\datatable
\begin{axis}[width=0.20\textwidth, xmin=-6,xmax=7,ymin=-5,ymax=8,                         xtick={-4,0,4},             ytick={-4,0,4}]
    \addplot[
        scatter/classes={0={backg}, 1={leftv}, 2={myo}, 3={rightv}},
        scatter, mark=*, only marks,
        mark options={xscale=0.5pt, yscale=0.5pt},
        scatter src=explicit symbolic,
        % nodes near coords*={\Label},
        visualization depends on={value \thisrow{label} \as \Label} %<- added value
    ] table [x index = 0, y index = 1, meta=label] {\datatable};
\end{axis}
\node[above,font=\scriptsize] at (current bounding box.north) {\hspace{3ex} + AFA (0.082)};
\end{tikzpicture}%
\begin{tikzpicture}
    \pgfplotstableread[col sep=comma]{figures/esoteric/pca/acdc/MixUp_AFA_esoteric_depth_0_pca.csv}\datatable
\begin{axis}[width=0.20\textwidth, xmin=-5,xmax=5,ymin=-5,ymax=5,                         xtick={-4,0,4},             ytick={-4,0,4}]
    \addplot[
        scatter/classes={0={backg}, 1={leftv}, 2={myo}, 3={rightv}},
        scatter, mark=*, only marks,
        mark options={xscale=0.5pt, yscale=0.5pt},
        scatter src=explicit symbolic,
        % nodes near coords*={\Label},
        visualization depends on={value \thisrow{label} \as \Label} %<- added value
    ] table [x index = 0, y index = 1, meta=label] {\datatable};
\end{axis}
\node[above,font=\scriptsize] at (current bounding box.north) {\hspace{3ex} + MixUp + AFA (0.122)};
\end{tikzpicture}

\begin{tikzpicture}
    \begin{customlegend}[legend columns=-1,legend style={draw=none,column sep=1ex},legend entries={\scriptsize Background, \scriptsize Left Ventricle, \scriptsize Myocardium, \scriptsize Right Ventricle}]
    \addlegendimage{only marks,mark=*,color=backg,fill}
    \addlegendimage{only marks,mark=*,color=leftv,fill}
    \addlegendimage{only marks,mark=*,color=myo,fill}
    \addlegendimage{only marks,mark=*,color=rightv,fill}
    \end{customlegend}
\end{tikzpicture}%

==> figures/esoteric/pca_p158_avg_transformed.tex <==
\definecolor{backg}{RGB}{42, 179, 205}
\definecolor{myo}{RGB}{250, 231, 35}
\definecolor{leftv}{RGB}{253, 127, 116}
\definecolor{rightv}{RGB}{150, 55, 173}
\begin{tikzpicture}
    \pgfplotstableread[col sep=comma]{figures/esoteric/pca/p158/No_Aug_esoteric_depth_0_pca.csv}\datatable
\begin{axis}[width=0.20\textwidth,
            xmin=-6,xmax=6,
            ymin=-3,ymax=8,
, xtick={-5,0,5}, ytick={-3,0,3,6}
]
    \addplot[
        scatter/classes={0={backg}, 1={leftv}, 2={myo}, 3={rightv}},
        scatter, mark=*, only marks, 
        mark options={xscale=0.5pt, yscale=0.5pt},
        scatter src=explicit symbolic,
        % nodes near coords*={\Label},
        visualization depends on={value \thisrow{label} \as \Label} %<- added value
    ] table [x index = 0, y index = 1, meta=label] {\datatable};
\end{axis}
\node[above,font=\scriptsize] at (current bounding box.north) {\hspace{3ex} No Aug. (0.033)};
\end{tikzpicture}%
\begin{tikzpicture}
    \pgfplotstableread[col sep=comma]{figures/esoteric/pca/p158/Base_esoteric_depth_0_pca.csv}\datatable
\begin{axis}[width=0.20\textwidth,
            xmin=-5,xmax=5,
            ymin=-3.5,ymax=3.5,
, xtick={-5,0,5}, ytick={-2,0,2}
]
    \addplot[
        scatter/classes={0={backg}, 1={leftv}, 2={myo}, 3={rightv}},
        scatter, mark=*, only marks, 
        mark options={xscale=0.5pt, yscale=0.5pt},
        scatter src=explicit symbolic,
        % nodes near coords*={\Label},
        visualization depends on={value \thisrow{label} \as \Label} %<- added value
    ] table [x index = 0, y index = 1, meta=label] {\datatable};
\end{axis}
\node[above,font=\scriptsize] at (current bounding box.north) {\hspace{3ex} Base (0.035)};
\end{tikzpicture}%
\begin{tikzpicture}
    \pgfplotstableread[col sep=comma]{figures/esoteric/pca/p158/MixUp_esoteric_depth_0_pca.csv}\datatable
\begin{axis}[width=0.20\textwidth,
            xmin=-6,xmax=6,
            ymin=-4,ymax=5,
, xtick={-5,0,5}, ytick={-2,0,2,4}
]
    \addplot[
        scatter/classes={0={backg}, 1={leftv}, 2={myo}, 3={rightv}},
        scatter, mark=*, only marks, 
        mark options={xscale=0.5pt, yscale=0.5pt},
        scatter src=explicit symbolic,
        % nodes near coords*={\Label},
        visualization depends on={value \thisrow{label} \as \Label} %<- added value
    ] table [x index = 0, y index = 1, meta=label] {\datatable};
\end{axis}
\node[above,font=\scriptsize] at (current bounding box.north) {\hspace{3ex} + MixUp (0.047)};
\end{tikzpicture}%
\begin{tikzpicture}
    \pgfplotstableread[col sep=comma]{figures/esoteric/pca/p158/AFA_esoteric_depth_0_pca.csv}\datatable
\begin{axis}[width=0.20\textwidth,
            xmin=-3,xmax=6,
            ymin=-3.5,ymax=5,
            xtick={-2,0,2,4}, ytick={-2,0,2,4}
]
    \addplot[
        scatter/classes={0={backg}, 1={leftv}, 2={myo}, 3={rightv}},
        scatter, mark=*, only marks,
        mark options={xscale=0.5pt, yscale=0.5pt},
        scatter src=explicit symbolic,
        % nodes near coords*={\Label},
        visualization depends on={value \thisrow{label} \as \Label} %<- added value
    ] table [x index = 0, y index = 1, meta=label] {\datatable};
\end{axis}
\node[above,font=\scriptsize] at (current bounding box.north) {\hspace{3ex} + AFA (0.040)};
\end{tikzpicture}%
\begin{tikzpicture}
    \pgfplotstableread[col sep=comma]{figures/esoteric/pca/p158/MixUp_AFA_esoteric_depth_0_pca.csv}\datatable
\begin{axis}[width=0.20\textwidth,
            xmin=-6,xmax=6,
            ymin=-2.5,ymax=3,
, xtick={-5,0,5}, ytick={-2,0,2}
]
    \addplot[
        scatter/classes={0={backg}, 1={leftv}, 2={myo}, 3={rightv}},
        scatter, mark=*, only marks,
        mark options={xscale=0.5pt, yscale=0.5pt},
        scatter src=explicit symbolic,
        % nodes near coords*={\Label},
        visualization depends on={value \thisrow{label} \as \Label} %<- added value
    ] table [x index = 0, y index = 1, meta=label] {\datatable};
\end{axis}
\node[above,font=\scriptsize] at (current bounding box.north) {\hspace{3ex} + MixUp + AFA (0.048)};
\end{tikzpicture}

\begin{tikzpicture}
    \begin{customlegend}[legend columns=-1,legend style={draw=none,column sep=1ex},legend entries={\small Background, \small Transition Zone, \small Peripheral Zone}
    % \small Right Ventricle}
    ]
    \addlegendimage{only marks,mark=*,color=backg,fill}
    \addlegendimage{only marks,mark=*,color=leftv,fill}
    \addlegendimage{only marks,mark=*,color=myo,fill}
    % \addlegendimage{only marks,mark=*,color=rightv,fill}
    \end{customlegend}
\end{tikzpicture}%

==> hacks/many-authors-hack.tex <==
% This hack should not be needed anynore as the issue has been fixed upstream in JMLR v1.26 (2020-01-31)
% https://github.com/MIDL-Conference/MIDLLatexTemplate/issues/8
% https://www.dickimaw-books.com/bugtracker.php?action=view&key=141

%\begin{comment}
\makeatletter
% hack the footer of the title page as it doesn't seem to automatically use the et al. version when spanning acros multiple pages
\renewcommand*{\@titlefoot}{\scriptsize\copyright\space\@jmlryear
    \ifanonsubmission
    \space Author(s) names withheld.\hfill
    \else
    \space \@firstauthor\space \emph{et al}.\hfill
    \@reprint
    \fi
  }
\makeatother
%\end{comment}

% \begin{comment}
\makeatletter
% remove the vbox in @jmlrmaketitle which prevents the text to be split across several pages
\renewcommand{\@jmlrmaketitle}{
  % specify the page style in case it spans over several pages. Not sure why this is needed
  \thispagestyle{jmlrtps}%
  % define a new label for the first page as otherwise it starts from 2 in the header
  \label{jmlrstartnew}%
  % hack the spacing to mimick what happens with a vbox
  \null\vspace{-\parindent}\vspace{-2pt}{
  \hsize\textwidth
  \linewidth\hsize
 \jmlrpretitle
  {%
    \def\titletag##1{##1}%
    \@title
  }%
 \jmlrposttitle
 \jmlrpreauthor \@author \jmlrpostauthor
}
% hack the spacing to mimick what happens with a vbox
\vspace{2pt}
}
\makeatother
%\end{comment}

%\begin{comment}
\makeatletter
% hack the footer to use the new counter
\renewcommand*\@jmlrpages{\pageref{jmlrstartnew}--\pageref{jmlrend}}
\makeatother
%\end{comment}

==> sections/preliminary.tex <==
% \section{Preliminary}

% moved to methodology

==> sections/related_works.tex <==
% Moved to Methodology

==> tables/all_metrics_ds.tex <==
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}ccc|c|cccccc|c|cc@{}}
\toprule
\multicolumn{3}{c}{Augmentation}          & \multicolumn{1}{|c|}{\multirow{2}{*}{\makecell{Trained \\ On}}}           & \multicolumn{3}{c}{ES} & \multicolumn{3}{c}{ED} & \multicolumn{1}{|c|}{\multirow{2}{*}{\makecell{Trained \\ On}}}        &    &    \\ \cmidrule(lr){1-3} \cmidrule(lr){5-7} \cmidrule(lr){8-10} \cmidrule(lr){12-13}
nnUNet       & MixUp        & AFA          &  & LV     & MYO     & RV    & LV     & MYO     & RV     &  & PZ & TZ \\ \midrule
$\checkmark$ &              &              & ACDC                        & 0.868  & 0.862 & 0.845 & 0.934  & 0.828  & 0.897 & MSD                         & 0.555 & 0.751 \\
$\checkmark$ & $\checkmark$ &              & ACDC                        & 0.886  & 0.870 & 0.849 & 0.939  & 0.835  & 0.903 & MSD                         & 0.595 & 0.816 \\
$\checkmark$ &              & $\checkmark$ & ACDC                        & 0.872  & 0.862 & 0.847 & 0.934  & 0.828  & 0.898 & MSD                         & 0.605 & 0.808 \\
$\checkmark$ & $\checkmark$ & $\checkmark$ & ACDC                        & 0.887  & 0.870 & 0.853 & 0.939  & 0.834  & 0.901 & MSD                         & 0.570 & 0.819 \\ \midrule
$\checkmark$ &              &              & MnMs                        & 0.886  & 0.867 & 0.860 & 0.939  & 0.839  & 0.910 & P158                        & 0.771 & 0.881 \\ \bottomrule
\end{tabular}
}


==> tables/all_metrics_results_acdc.tex <==
\begin{tabular}{ccclllllllccllllllc}
\toprule
\multicolumn{3}{c}{\multirow{2}{*}{Augmentation}}                       & \multicolumn{16}{c}{ACDC}                                                                                                                                        \\ 
\multicolumn{3}{c}{}                                                    & \multicolumn{8}{c}{Original}                                                 & \multicolumn{8}{c}{Transformed}                                                   \\ \midrule
\multirow{2}{*}{nnUNet} & \multirow{2}{*}{MixUp} & \multirow{2}{*}{AFA} & \multicolumn{4}{c}{DSC}      & \multicolumn{4}{c}{HD95}                      & \multicolumn{4}{c}{DSC}                 & \multicolumn{4}{c}{HD95}                \\
                        &                        &                      & S1    & S2    & S3    & avg. & S1   & S2   & S3   & \multicolumn{1}{l}{avg.} & \multicolumn{1}{l}{S1} & S2 & S3 & avg. & S1 & S2 & S3 & \multicolumn{1}{l}{avg.} \\ \midrule
                        &                        &                      & 0.880 () & 0.877 () & 0.915 () &      & 7.07 () & 4.72 () & 5.63 () &                          &                        &    &    &      &    &    &    &                          \\
                        & $\checkmark$           &                      & 0.880 () & 0.873 () & 0.914 () &      & 6.98 () & 5.37 () & 5.89 () &                          &                        &    &    &      &    &    &    &                          \\
                        &                        & $\checkmark$         & 0.858 () & 0.843 () & 0.899 () &      & 7.94 () & 5.59 () & 5.93 () &                          &                        &    &    &      &    &    &    &                          \\
                        & $\checkmark$           & $\checkmark$         & 0.870 () & 0.856 () & 0.903 () &      & 7.19 () & 5.74 () & 6.11 () &                          &                        &    &    &      &    &    &    &                          \\ \midrule
$\checkmark$            &                        &                      & 0.921 () & 0.909 () & 0.946 () &      & 4.30 () & 2.85 () & 2.97 () &                          &                        &    &    &      &    &    &    &                          \\
$\checkmark$            & $\checkmark$           &                      & 0.921 () & 0.910 () & 0.942 () &      & 4.26 () & 2.95 () & 3.26 () &                          &                        &    &    &      &    &    &    &                          \\
$\checkmark$            &                        & $\checkmark$         & 0.916 () & 0.904 () & 0.939 () &      & 4.32 () & 3.10 () & 3.76 () &                          &                        &    &    &      &    &    &    &                          \\
$\checkmark$            & $\checkmark$           & $\checkmark$         & 0.917 () & 0.906 () & 0.940 () &      & 4.46 () & 3.04 () & 3.30 () &                          &                        &    &    &      &    &    &    &                          \\ \bottomrule
\end{tabular}


==> tables/all_metrics_results_p158.tex <==
\begin{tabular}{cccllllllllllll}
\toprule
\multicolumn{3}{c}{\multirow{2}{*}{Augmentation}}                       & \multicolumn{12}{c}{P158}                                                                               \\
\multicolumn{3}{c}{}                                                    & \multicolumn{6}{c}{Original}                       & \multicolumn{6}{c}{Transformed}                    \\ \midrule
\multirow{2}{*}{nnUNet} & \multirow{2}{*}{MixUp} & \multirow{2}{*}{AFA} & \multicolumn{3}{c}{DSC} & \multicolumn{3}{c}{HD95} & \multicolumn{3}{c}{DSC} & \multicolumn{3}{l}{HD95} \\
                        &                        &                      & S1    & S2    & Avg.    & S1     & S2    & Avg.    & S1    & S2    & Avg.    & S1     & S2    & Avg.    \\ \midrule
                        &                        &                      & ()    & ()    & ()      & ()     & ()    & ()      & ()    & ()    & ()      & ()     & ()    & ()      \\
                        & $\checkmark$           &                      & ()    & ()    & ()      & ()     & ()    & ()      & ()    & ()    & ()      & ()     & ()    & ()      \\
                        &                        & $\checkmark$         & ()    & ()    & ()      & ()     & ()    & ()      & ()    & ()    & ()      & ()     & ()    & ()      \\
                        & $\checkmark$           & $\checkmark$         & ()    & ()    & ()      & ()     & ()    & ()      & ()    & ()    & ()      & ()     & ()    & ()      \\ \midrule
$\checkmark$            &                        &                      & ()    & ()    & ()      & ()     & ()    & ()      & ()    & ()    & ()      & ()     & ()    & ()      \\
$\checkmark$            & $\checkmark$           &                      & ()    & ()    & ()      & ()     & ()    & ()      & ()    & ()    & ()      & ()     & ()    & ()      \\
$\checkmark$            &                        & $\checkmark$         & ()    & ()    & ()      & ()     & ()    & ()      & ()    & ()    & ()      & ()     & ()    & ()      \\
$\checkmark$            & $\checkmark$           & $\checkmark$         & ()    & ()    & ()      & ()     & ()    & ()      & ()    & ()    & ()      & ()     & ()    & ()      \\ \bottomrule
\end{tabular}


==> tables/avg_metrics_supp_ds.tex <==
\resizebox{\textwidth}{!}{%
\begin{tabular}{ccccccccc}
\toprule
\multicolumn{3}{c}{Augmentation}          & \multicolumn{3}{c}{Cardiac Cine MR} & \multicolumn{3}{c}{Prostate bpMRI} \\ \cmidrule{1-3} \cmidrule(lr){4-6} \cmidrule(lr){7-9}
nnUNet       & MixUp        & AFA          & Trained On   & DSC     & HD95 (mm)   & Trained On   & DSC    & HD95 (mm)  \\ \midrule
$\checkmark$ &              &              & \multirow{4}{*}{ACDC}         & 0.870   & 7.97        &  \multirow{4}{*}{MSD}         & 0.653  & 10.14      \\
$\checkmark$ & $\checkmark$ &              &                        & {\color[HTML]{3233B9} 0.880} & {\color[HTML]{3233B9} 5.74} &                       & {\color[HTML]{3233B9} 0.705} & {\color[HTML]{3233B9} 9.29} \\
$\checkmark$ &              & $\checkmark$ &                        & {0.874} & {6.92} &                       & {\color[HTML]{3233B9} 0.706} & {\color[HTML]{3233B9} 9.39} \\
$\checkmark$ & $\checkmark$ & $\checkmark$ & \multirow{-4}{*}{ACDC} & {\color[HTML]{3233B9} 0.880} & {\color[HTML]{3233B9} 5.70} & \multirow{-4}{*}{MSD} & {\color[HTML]{3233B9} 0.695} & {\color[HTML]{3233B9} 9.60} \\ \midrule
$\checkmark^\dagger$ &              &              & M\&Ms        & 0.882   & 5.08        & P158         & 0.825  & 4.60       \\ \bottomrule
\end{tabular}
}
